The Likelihood Ratio Test in High-Dimensional Logistic Regression Is Asymptotically a Rescaled Chi-Square

Logistic regression is used thousands of times a day to fit data, predict future outcomes, and assess the statistical significance of explanatory variables. When used for the purpose of statistical inference, logistic models produce p-values for the regression coefficients by using an approximation to the distribution of the likelihood-ratio test. Indeed, Wilks' theorem asserts that whenever we have a fixed number $p$ of variables, twice the log-likelihood ratio (LLR) $2\Lambda$ is distributed as a $\chi^2_k$ variable in the limit of large sample sizes $n$; here, $k$ is the number of variables being tested. In this paper, we prove that when $p$ is not negligible compared to $n$, Wilks' theorem does not hold and that the chi-square approximation is grossly incorrect; in fact, this approximation produces p-values that are far too small (under the null hypothesis). Assume that $n$ and $p$ grow large in such a way that $p/n\rightarrow\kappa$ for some constant $\kappa < 1/2$. We prove that for a class of logistic models, the LLR converges to a rescaled chi-square, namely, $2\Lambda~\stackrel{\mathrm{d}}{\rightarrow}~\alpha(\kappa)\chi_k^2$, where the scaling factor $\alpha(\kappa)$ is greater than one as soon as the dimensionality ratio $\kappa$ is positive. Hence, the LLR is larger than classically assumed. For instance, when $\kappa=0.3$, $\alpha(\kappa)\approx1.5$. In general, we show how to compute the scaling factor by solving a nonlinear system of two equations with two unknowns. Our mathematical arguments are involved and use techniques from approximate message passing theory, non-asymptotic random matrix theory and convex geometry. We also complement our mathematical study by showing that the new limiting distribution is accurate for finite sample sizes. Finally, all the results from this paper extend to some other regression models such as the probit regression model.

==> setup.tex <==
\section{The problem}\label{sec: problem}
This paper focuses on binary regression. Consider $n$ independent observations $\{y_i,\bX_i\}_{1\leq i\leq n}$, such that $y_i \in \{0,1 \}$ and $\bX_i \in \R^{p}$. In the framework of GLMs, it is assumed that $y_i$'s are drawn from a generalized linear model (GLM)   with natural parameter $\eta_i$ and probability mass function given by \cite{GLM89}
\begin{equation}
  \label{eq:GLM-density}
  g_{\eta_i}(y_i) = \exp \big\{\eta_i y_i - \rho(\eta_i) \big\}, 
\end{equation}
where $\rho(\cdot)$ is the link function. For GLMs, the natural parameter $\bm{\eta}=[\eta_1,\cdots, \eta_n]^{\top}$ is assumed to satisfy the following form
\begin{equation}
  \eta_i = f( \bX_i^{\top}\bbeta), \quad i = 1,\cdots,n, 
\end{equation}
%\begin{equation}
%  \bm{\eta} = \bX\bbeta,
%\end{equation}
for some specified function $g$, where $\bm{X} = [\bm{X}_1,\cdots,\bm{X}_n]^{\top} \in \mathbb{R}^{n\times p}$ is a known design matrix and  $\bbeta=[\beta_1,\cdots,\beta_p]^{\top}$ represents the unknown parameters. Under such models, the maximum likelihood estimate (MLE) can  be computed by solving
\begin{equation}
\underset{{\bm{\beta}\in\mathbb{R}^{p}}}{\text{minimize}}\quad\ell\left(\bm{\beta}\right):=\sum_{i=1}^{n}\left\{ -y_{i}f(\bm{X}_{i}^{\top}\bm{\beta})+\rho\left(\bm{X}_{i}^{\top}\bm{\beta}\right)\right\},
\label{eq:MLE}
\end{equation}
where $\ell(\bm{\beta})$ is the {\em negative} log-likelihood function.

The goal of this work is to analyze the distribution of the {\em likelihood ratio test} (LRT) statistic, for testing for the $j$-th coefficient, $\beta_j=0$ against the alternative $\beta_j \neq 0$ under certain conditions, in the high dimensional regime where the number $p$ of covariates grows proportionally with the number $n$ of observations; specifically, we assume 
\begin{equation}
  \label{defn:kappa}
  \frac{p}{n} \rightarrow \kappa
\end{equation}
as $n$ diverges to infinity, where $\kappa \in (0,\delta)$ is a fixed constant independent of $n$ and $p$ and $\delta = 0.5 -\epsilon$ for a sufficiently small $\epsilon > 0$ which we will specify later. This condition is enforced simply to ensure the existence of the MLE and to guard against the separation issue in logisitc regression. 
\ps{ELABORATE ON THE SEPARATION ISSUE HERE.} 

%\yxc{I guess $\kappa \in (0,~0.5)$ is perhaps only relevant for special cases like logistic regression?}. 

Further, assume that the entries of $\bX=[X_{i,j}]_{1\leq i\leq n,1\leq j\leq p}$ are i.i.d.~obeying
\begin{equation}
  X_{i,j} \sim \mathcal{N}(0,1)
\end{equation}
and that the global null is true, that is, the true unknown satisfies $\bbeta = \bzero$. Under these assumptions, we aim to characterize the asymptotic distribution of the LRT statistic for binary regression with certain assumptions on the functions $f$ and $\rho$.\ps{Detail the assumptions in the assumptions section and refer to that or detail them here}. Our findings reveal that the asymptotic behavior of the LRT is quite different from classical results. (\ps{Details of discussion of classical results will go in the introduction}). %(\yxc{We should discuss classical results somewhere}). 

In particular, our results are applicable to binary regression with the following two simple yet most widely used link functions \cite{agresti2011categorical}:
\begin{itemize}
  \item[1)] The logistic model, where 
  %$y_i \sim \dber(p_i)$,
  \begin{equation}
  f(x)=x, \qquad 
     \rho(x)=\log(1+e^{x}) \qquad \text{and} \qquad
     y_i = \begin{cases} 1, & \text{w.p. } \frac{e^{\bX_i^{\tp}\bbeta}}{1+e^{\bX_i^{\tp}\bbeta}}, \\
     0, & \text{else.}\end{cases}
   %g_{\eta_i}(y_i) =p_i^{y_i}(1-p_i)^{1-y_i}. 
   \label{eq:logistic-link} 
\end{equation}
Note that here $\rho''(\eta)=\frac{e^\eta}{(1+e^{\eta})^2}$. \ps{Should we keep this derivative here or not.}
  \item[2)] The probit model, where 
  \begin{equation}\label{eq:probit-link}
  f(x)=\log \left(\frac{\Phi(x)}{1-\Phi(x)}\right), \ \ 
    \rho(x) =-\log(1-\Phi(x))\ \ \text{and} \ \ y_i = \begin{cases} 1, & \text{w.p. } \Phi(\bX_i^{\tp}\bbeta), \\
     0, & \text{else.}\end{cases}
  \end{equation}
 with $\Phi$ the cumulative distribution function (CDF) of a standard normal.  
 %Hence in this case the link function is given by  The derivatives of the link are $\rho'(\eta) = \Phi(\eta) $ and $\rho''(\eta)=\phi(\eta):=\frac{1}{\sqrt{2\pi}}\exp(-\eta^2/2)$. 

  %\item[3)] The complementary log-log (CLogLog) model, where the link function obeys
   %\begin{equation}
      %'(\eta) = 1- e^{-e^ \eta}.
   %\end{equation}
\end{itemize}

%In all the three cases above, the derivatives of the link $\rho'$ and $\rho''$ are non-negative and bounded.

Under the global null, in either of these two cases, $y_i \iid \dber(1/2)$. 

We would like to introduce some notations here. Denote $Y$ to be a random variable independent of all other random variables we consider here, drawn from the common distribution of $y_i$ for any $i$. (Note under global null, all $y_i$'s have the same distribution.) Let $\opP_Y$ refer to its pmf. Let $Z \sim \dnorm(0,1)$, independent of all other random variables considered.

An interval written as $(a,b)$ always refers to $(\min(a,b),\max(a,b)).$ 
%\yxc{Why do we need this?}

Here we are interested in establishing the asymptotic distribution of the LRT statistic for the individual coefficients $\beta_j$ for any $j \in \{1,\hdots,p\}$. Under the global null, they should have the same distribution . Hence, it suffices to characterize the distribution for testing one particular coefficient. We fix the first variable and characterize the LRT distribution for testing $\beta_1=0$ vs $\beta_1 \neq 0$. Throughout we need to define analogous variables for the full model with $p$ variables, and for the restricted model with $p-1$ variables, formed by dropping the first column of $\bX.$ These variables will be denoted by same notation without and with tilde respectively. For example, $\bX$ is the design matrix for the full model and $\tbX$ the design matrix for the restricted model obtained by dropping the first column of  $\bX$. The $i$-th row of $\bX$ is $\bX_i^{\tp}$. The MLE is denoted by $\hbbeta$ and $\tbbeta$ for the full and restricted model,  respectively. 

Any mention of $C$ or $C_i$ for $i \in \mathbb{N}$ refers to some positive universal constant appropriate in the relevant context and the constant can change from line to line. For a square symmetric matrix $\bM$ the minimum eigenvalue is denoted by $\lambda_{\min}(\bM)$. 


